Accelerating Real-Time Question Answering via Question Generation

Although deep neural networks have achieved tremendous success for question answering (QA), they are still suffering from heavy computational and energy cost for real product deployment. Further, existing QA systems are bottlenecked by the encoding time of real-time questions with neural networks, thus suffering from detectable latency in deployment for large-volume traffic. To reduce the computational cost and accelerate real-time question answering (RTQA) for practical usage, we propose to remove all the neural networks from online QA systems, and present Ocean-Q (an Ocean of Questions), which introduces a new question generation (QG) model to generate a large pool of QA pairs offline, then in real time matches an input question with the candidate QA pool to predict the answer without question encoding. Ocean-Q can be readily deployed in existing distributed database systems or search engine for large-scale query usage, and much greener with no additional cost for maintaining large neural networks. Experiments on SQuAD(-open) and HotpotQA benchmarks demonstrate that Ocean-Q is able to accelerate the fastest state-of-the-art RTQA system by 4X times, with only a 3+% accuracy drop.

==> Ocean-Q NAACL2021/exp.tex <==
\section{Experiments}

\subsection{Experimental Setup}
\paragraph{Datasets} We conduct experiments on SQuAD~\cite{rajpurkar-etal-2016-squad} and HotpotQA~\cite{yang2018hotpotqa} to validate the effectiveness of our proposed approach.
SQuAD is one of the largest QA datasets that requires mostly single-hop reasoning, while HotpotQA is a popular benchmark for multi-hop QA. Both are collected over 100K questions by presenting a set of Wikipedia articles to crowdworkers. 

\paragraph{Metrics} For RTQA evaluation, we follow DENSPI~\cite{denspi} to compare EM, F1 and inference speed (s/Q) on open-domain SQuAD (SQuAD-Open) and SQuAD v1.1 development sets as our test sets. The answer extraction and QA-pair verification models are trained on the original SQuAD v1.1 training set. 
The question generation model is trained on SQuAD, HotpotQA and NewsQA datasets through multi-task learning. 

For QG evaluation, we follow~\citet{du-cardie-2018-harvesting} to split the original training set into training and test on SQuAD, and follow~\citet{pan-etal-2020-DQG} to use their released data split for a fair comparison on HotpotQA.
Besides commonly used metrics such as BLEU-4, METEOR and ROUGE-L, we also use final RTQA performance to measure QG quality.
Since~\citet{pan-etal-2020-DQG} pre-processes the original HotpotQA dataset to select relevant sentences because of the difficulty in producing accurate semantic graphs for very long documents, %\jj{What purpose?} 
the RTQA score on HotpotQA is based on the evidence sentences rather than the whole context. 
%Implementation details can be found in appendix~\ref{appendix:implementation}.

\paragraph{Implementation Details} Our implementation is mainly based on HuggingFace's Transformers~\cite{Wolf2019HuggingFacesTS}, UniLM~\cite{unilm} and DrQA~\cite{chen2017reading}. We conduct experiments on 16 NVIDIA V100 GPUs and Intel(R) Xeon(R) W-2175 CPU.
Each model in Ocean-Q framework took several hours to finetune.
For offline QA-pair generation from Wikipedia, it took about one week. Datasets and more implementation details can be found in the Appendix. %~\ref{appendix:dataset} and ~\ref{appendix:implementation}.

\subsection{Real-Time QA Experiments}

\begin{table}[t!]
%\small
\centering
%\begin{adjustbox}{scale=0.90,center}
\resizebox{1.0\columnwidth}{!}{
\begin{tabular}{lcccc}
\toprule
 & Parameters & EM & F1 & s/Q \\
 \midrule
DrQA & 68M & 29.8 & - & 35\\
R$^3$ & - &  29.1 & 37.5 & - \\
Paragraph ranker & 68M &  30.2 & - & - \\
Multi-step reasoner & 68M &  31.9 & 39.2 & - \\
MINIMAL & - &  34.7 & 42.5 & - \\
BERTserini & 110M &  38.6 & 46.1 & 115 \\
Weaver & - & -  & 42.3 &  - \\
%Multi-passage BERT & 53.0 & 60.9 &  84 & 30 \\
%DENSPI-SFS & 33.3 & 42.5 & 1.03$^*$ & 5 \\
%DENSPI-DFS & 28.5 & 35.9 & 0.94$^*$ & 815 \\
DENSPI-Hybrid & 336M & 36.2 & 44.4 & 1.24$^*$ \\ \midrule
%DENSPI-Hybrid + Sparc & 40.7 & 49.0 & 1.21 & 817 \\ \hline
Ocean-Q & 0 & 32.7 & 39.4 &  0.28 \\
\bottomrule
\end{tabular}
}
%\end{adjustbox}
\caption{\label{table:SQuAD-open} Results on SQuAD-open. `s/Q' is the average seconds per query in CPU environment. 
%and `\#D/Q' is the number of documents used per query.
Note that DENSPI does not include the inference time of question embedding in their evaluation. We used their code to load question embedding on the dev set, which cost 0.43 seconds on average and was added to their reported numbers, marked as asterisk (*).}
\label{sec:exp-sta}
\end{table}

\begin{table}[t!]
\centering
\begin{adjustbox}{scale=0.90,center}
%\resizebox{1.0\columnwidth}{!}{
\begin{tabular}{cccc}
\toprule
 & Model & EM & F1 \\
 \midrule
\multirow{2}{*}{Original} & DrQA & 69.5 & 78.8 \\
& BERT & 84.1 & 90.9 \\ \midrule
\multirow{3}{*}{\shortstack{Query-\\Agnostic}} & LSTM+SA+ELMo & 52.7 & 62.7 \\ 
& DENSPI  & 73.6 & 81.7 \\ 
& Ocean-Q & 63.0 & 70.5 \\ \bottomrule
\end{tabular}
%}
\end{adjustbox}
\caption{Results on SQuAD v1.1. DrQA~\cite{chen2017reading} and BERT~\cite{devlin2018bert} results are reported by SQuAD leaderboard. LSTM+SA+ELMo~\cite{seo2018phrase} and DENSPI~\cite{denspi} are two query-agnostic baselines.}
\label{table:SQuAD-close}
\vspace{-10pt}
\end{table}
\label{sec:exp-qa}

\paragraph{Baselines} 
On SQuAD-Open, state-of-the-art (SOTA) models include DrQA~\cite{chen2017reading}, R$^3$~\cite{wang2018r}, Paragraph ranker~\cite{lee2018ranking}, Multi-step reasoner~\cite{das2019multi}, MINIMAL~\cite{min2018efficient}, BERTserini~\cite{yang2019end}, Weaver~\cite{raison2018weaver} and DENSPI~\cite{denspi}. 
On SQuAD v1.1, we follow~\citet{denspi} to compare with two types of model. The first group includes DrQA~\cite{chen2017reading} and BERT~\cite{devlin2018bert} that rely on cross attention between the question and context. 
The second group includes LSTM+SA+ELMO~\cite{seo2018phrase} and DENSPI~\cite{denspi} as query-agnostic models. 
The accuracy comparison in following experiments is based on subtracting the EMs from two comparing systems.

\paragraph{Results}
Table~\ref{table:SQuAD-open} and~\ref{table:SQuAD-close} summarize results on SQuAD-Open and SQuAD v1.1 datasets.
In open domain setting:
$(i)$ Ocean-Q outperforms DrQA by 3\% and achieves 125x speedup.
This indicates that Ocean-Q could outperform earlier cross-attention model while achieving much faster inference speed.
$(ii)$ Compared to BERTserini, Ocean-Q achieves 410 times speedup while sacrificing accuracy by 5.8\%.
As pointed out in~\citet{denspi}, the main gap between query-agnostic model and cross-sequence attention model is due to the \emph{decomposability gap}.
$(iii)$ Ocean-Q accelerates DENSPI by 4 times at the expense of 3.5\% accuracy drop.
We call this gap the \emph{generative gap}, since Ocean-Q relies on question generation model to enumerate possible questions for RTQA. A more rigorous QG model design to generate more diverse questions may help close this gap.
In close-domain setting (a simpler problem than open domain), Table~\ref{table:SQuAD-close} shows that Ocean-Q outperforms the query-agnostic baseline~\cite{seo2018phrase}, which drops 30.3\% from close- to open-domain; while DENSPI, BERT and DrQA drop 37.4\%, 45.5\%, and 39.7\%, respectively.
This demonstrates Ocean-Q's better generalization ability from close- to open-domain.

\subsection{Question Generation Experiments}
\label{subsec:qg-exp}

%In this subsection, we experiment with three different methods to enhance QG model for further boosting RTQA performance.
\begin{table}[t!]
%\small
\centering
%\begin{adjustbox}{scale=0.9,center}
\resizebox{1.0\columnwidth}{!}{
\begin{tabular}{lccccc}
\toprule
& \multicolumn{3}{c}{QG} & \multicolumn{2}{c}{RTQA} \\
& BLEU-4 & MTR & RG-L & EM & F1 \\ \midrule
\multicolumn{6}{l}{\emph{SQuAD}} \\ \midrule
CorefNQG & 15.16 & 19.12 & - & - & - \\
SemQG & 18.37 & 22.65 & 46.68 & - & - \\
UniLM & 22.78 & 25.49 & 51.57 & - & - \\
UniLMv2 & 24.70 & 26.33 & 52.13 & - & - \\
Our baseline & 22.89 & 25.46 & 51.52 & 62.33 & 70.09 \\
+ DA-sim & 23.72 & 26.07 & 52.23 & 62.03 & 69.68 \\
+ DA-div & 22.15 & 25.13 & 51.29 & 62.71 & 70.34 \\
+ MTL & 23.16 & 25.74 & 51.94 & 63.04 & 70.52 \\
%+ DBS & 22.89 & 25.46 & 51.52 & - & - \\
+ DBS & 22.89 & 25.46 & 51.52 & 62.43 & 70.26  \\ \midrule
\multicolumn{6}{l}{\emph{HotpotQA}} \\ \midrule
SRL-Graph & 15.03 & 19.73 & 36.24 & - & - \\
DP-Graph & 15.53 & 20.15 & 36.94 & - & - \\
Our baseline & 26.46 & 26.75 & 46.64 & 42.93 & 54.18 \\
+ DA-sim & 28.53 & 28.36 & 48.78 & 44.39 & 55.79 \\
+ DA-div & 26.94 & 27.27 & 47.18 & 44.19 & 55.43 \\ 
+ MTL & 26.76 & 27.03 & 46.97 & 44.30 & 55.73 \\
%+ DBS & 26.46 & 26.75 & 46.64 & - & - \\
+ DBS & 26.46 & 26.75 & 46.64 & 43.53 & 54.91 \\
%+ Nucleus p & - & - & - & - & - \\
\bottomrule
\end{tabular}
}
%\end{adjustbox}
\caption{\label{table:QG-QA} Results of QG Enhancement on SQuAD and HotpotQA. The first group follows the data split in~\citet{du-cardie-2018-harvesting} on SQuAD, while the second group follows~\citet{pan-etal-2020-DQG} on HotpotQA. MTR is short for METEOR, and RG-L for ROUGE-L.}
\vspace{-10pt}
\end{table}

\begin{table*}[t!]
\centering
\begin{small}
\begin{tabular}{lll}
\toprule
\textbf{Passage} & \multicolumn{2}{p{0.85\textwidth}}{\textcolor{blue}{Super Bowl 50} was an American football game to determine ... The \textcolor{blue}{American Football Conference (AFC)} champion \textcolor{blue}{Denver Broncos} defeated the \textcolor{blue}{National Football Conference (NFC)} champion \underline{\textcolor{blue}{Carolina Panthers 24-10}} to earn their third \textcolor{blue}{Super Bowl} title. The game was played on ... }\\
%\multirow{4}{*}{\textbf{Passage}} & \multicolumn{2}{l}{}
\textbf{QA Pairs} & What was the winning score in the Super Bowl? & 24-10 \\
%& What was the outcome of the Super Bowl? & 24-10 \\
& \textcolor{red}{What was the final score of the Super Bowl?} &  \textcolor{red}{24-10} \\
%& What was the final score in the Super Bowl? & 24-10 \\
& Who did the Denver Broncos defeat in the Super Bowl? & Carolina Panthers \\
%& ...  \\
\textbf{Question} & What was the final score of Super Bowl 50? & \\ 
\midrule
\textbf{Passage} & \multicolumn{2}{p{0.85\textwidth}}{Demographically, it was the most diverse city in \textcolor{blue}{Poland}, with significant numbers of \textcolor{blue}{foreign-born inhabitants}. … In \textcolor{blue}{1933}, out of \underline{\textcolor{blue}{1,178,914}} inhabitants \textcolor{blue}{833,500} were of \textcolor{blue}{Polish mother tongue}. \textcolor{blue}{World War II} changed the demographics of the city, and to this day ...} \\
\textbf{QA Pairs} & What was the population of Warsaw in 1933? & 1,178,914 \\
%& How many people lived in Warsaw in 1933? & 1,178,914 \\
%& In 1933 , how many people lived in Warsaw? & 1,178,914 \\
& How many people in 1933 had Polish mother tongue? & 833,500 \\
& \textcolor{red}{How many inhabitants in 1933 had Polish mother tongue?} & \textcolor{red}{833,500} \\
%& ... \\
\textbf{Question} & How many of Warsaw's inhabitants spoke Polish in 1933? & \\
\bottomrule
\end{tabular}
\end{small}
\caption{Qualitative examples of generated QA pairs and predictions. {\color{blue}Blue} and {\color{red} red} represent the extracted answers and matched QA pair. Sampled QA pairs generated by Ocean-Q correspond to the \underline{\textcolor{blue}{underline}} answer span.}
\label{tab:examples}
\vspace{-5pt}
\end{table*}

\paragraph{Baselines}
On SQuAD, we compare with SOTA baselines: CorefNQG~\cite{du-cardie-2018-harvesting}, SemQG~\cite{zhang-bansal-2019-addressing}, UniLM~\cite{unilm} and UniLMv2~\cite{unilmv2}. 
On HotpotQA, our chosen baselines are SRL-Graph~\cite{pan-etal-2020-DQG} and DP-Graph~\cite{pan-etal-2020-DQG}. 
We reproduced the results from the released SOTA model UniLM and used this as our baseline.

\paragraph{Results}
Table~\ref{table:QG-QA} compares Ocean-Q with baselines over QG metrics as well as final RTQA scores.
For data augmentation (DA), We use two different F1 thresholds. One from 0.5 to 1.0 (DA-sim) is intended to select similar questions, while the other one from 0.0 to 0.5 (DA-div) tends to select more diverse questions.
Our observations from the comparison results:
$(i)$ DA-div, multi-task learning (MTL) and diverse beam search (DBS) improve RTQA score by 0.38/0.71/0.10 and 1.26/1.37/0.60 points, respectively, over the baseline on SQuAD and HotpotQA.
This indicates that diversified questions could be beneficial for lifting RTQA performance.
$(ii)$ DA improves 0.83/0.61/0.71 and 2.07/1.61/2.14 points, respectively, over our strong baseline on SQuAD and HotpotQA.
Compared to current SOTA, it still falls behind by 0.98/0.26/0.10 points over UniLMv2 on SQuAD, but it significantly boosts 13.0/8.21/11.84 points over DP-Graph on HotpotQA.
$(iii)$ MTL improves the most for RTQA, and DA improves the most on QG metrics.
This indicates that RTQA benefits more from out-of-domain data, while QG metrics gain more from in-domain data. 
$(iv)$ Similar in-domain data help more on QG metrics than diverse data.
Comparing DA-sim with our baseline, it improves 0.83/0.61/0.71 and 2.07/1.61/2.14 points on SQuAD and HotpotQA, respectively. In contrast, DA-div is worse than the baseline on SQuAD and achieves less gain on HotpotQA.
%(2) RTQA score might reflect better in terms of the generalization of QG model.
%Compared with data augmentation, multi-task learning improves less on QG scores, but helps more on downstream QA task.
%Consider multitask learning might generalize better than in-domain data augmentation since it uses out-of-domain data, the RTQA score is more consistent with its improvement.
%(3) More diverse questions could help improving RTQA.
%Compared with our baseline, diverse beam search could further improve RTQA score by 0.50/0.55 points due to the more diverse N-best list while QG scores are same as baseline since they only measure the 1-best sequence.
%Overall, our RTQA score reflects better than QG metrics in terms of measuring the generalization and diversity of QG model for downstream QA task.

\begin{figure}[t!]
\centering
{\includegraphics[width=\linewidth]{images/ans_beam.png}}
\caption{\label{fig:effects_ans_beam} Effects of increasing the number of candidate answers and beam size on SQuAD RTQA performance. When answer number is 100 and beam size is 20, the setting degenerates to our baseline in Table~\ref{table:QG-QA}.}
\vspace{-10pt}
\end{figure}

%\begin{figure}[t!]
%\centering
%{\includegraphics[width=\linewidth]{beam_size.png}}
%\caption{\label{fig:beam_size} Effects of increasing beam size.}
%\end{figure}


% \begin{table}[t!]
%\small
%\centering
%\begin{adjustbox}{scale=0.95,center}
%\begin{tabular}{lcc}
%\hline
%& EM & F1 \\ \hline
%our baseline & 62.33 & 70.09 \\
%- QA Pair Verification & 41.81 & 60.63 \\ \hline
%\end{tabular}
%\end{adjustbox}
%\caption{\label{table:abl-verify} Ablation study of QA Pair Verification on SQuAD Dev.}
%\end{table}

\begin{table}[t!]
%\small
\centering
\begin{adjustbox}{scale=0.90,center}
%\resizebox{1.0\columnwidth}{!}{
\begin{tabular}{cccc}
\toprule
%Retriever & \#paras & \#paras/Q & Accuracy(\%) \\
Retriever & \#Docs & \#Paras & Accuracy(\%) \\
 \midrule
DrQA & 5 & 214 & 77.8 \\ \midrule
\multirow{3}{*}{\shortstack{Two-step\\Ranker}} & 20 & 100 & 80.6 \\
%20 & 10 & 59.8 \\
%& 20 & 50 & 76.3 \\
& 20 & 150 & 82.4 \\
& 20 & 200 & 83.4 \\
% & 20 & 71 & 83.4 \\
\bottomrule
\end{tabular}
%}
\end{adjustbox}
\caption{\label{table:eff_ranker}Paragraph retrieval results on SQuAD-Open.
`\#Docs' and `\#Paras' are the number of retrieved document and paragraph per query. `Accuracy' is the percentage of questions whose answers appear in the retrieved paragraphs. DrQA~\cite{chen2017reading} retrieves 5 documents for each question. 
For the two-step ranker, we retrieve 100, 150 and 200 paragraphs from 20 Wikipedia documents for each question.}
%\vspace{-10pt}
\end{table}


\subsection{Analysis}
We provide four analysis to evaluate the effectiveness of each component in Ocean-Q framework: $(i)$ Effect of different numbers of candidates in answer extraction; $(ii)$ Effect of beam size in question generation; $(iii)$ Ablation on QA pair verification; and (iv) Effect of the two-step ranker in online question matching. 
Figure~\ref{fig:effects_ans_beam} show that RTQA score receives consistent improvement by increasing the number of candidate answers and beam search size, since both methods generate more diverse candidate question-answer pairs. By increasing the answer number from 10 to 100, RTQA score receives 16.96/18.85 points improvement. By enlarging beam size from 1 to 20, there is 12.02/11.59 points improvement. 
For QA-pair verification, we see 9.46\% accuracy drop if ablating this step in the experiment, which demonstrates that QA pair verification is useful for improving RTQA performance.
For two-step ranker, Table~\ref{table:eff_ranker} shows that by using the ranker, our model achieves 5.6\% higher accuracy than DrQA using similar number of paragraphs (200 vs. 214), and 2.8\% higher using just half (100 vs. 214).
%\vspace{-5pt}

\paragraph{Qualitative Analysis}
Table~\ref{tab:examples} shows two qualitative examples of generated QA pairs and predictions by Ocean-Q. 
In the first example, the extracted answer span ``Carolina Panthers 24-10'' includes two possible sub answers ``Carolina Panthers'' and ``24-10''.
This phenomena is expected since the answer extraction model cannot precisely know where is the answer boundary.
However, QG model can generate different questions through attention over different sub answers, and the QA verification model can further correct inaccurate answers from the answer extraction phase.
In the second example, we note that the same input answer span ``1,178,914'' generates questions that correspond to different spans in the passage. 
We hypothesize that since ``1,178,914'' and ``833,500'' appear close to each other in the passage, QG model may not distinguish them from the context and thus generate inaccurate questions.
But the QA verification model can help correcting the false answer.
%\vspace{-5pt}

\paragraph{Green NLP Analysis} As shown in Table~\ref{sec:exp-sta}, we are the first method that can answer questions without using neural networks. 
Usually, models with more parameters can achieve better performance, especially when they are initialized by pre-trained models.
Our model without neural networks during inference can achieve very competitive performance.
Compared to the baseline of DENSPI, we both need to save a large amount of answer candidates into disk. 
However, DENSPI still needs to compute the question embedding whenever a new question comes in.
Our method does not require a heavy computational cost from neural networks, but only the information retrieval cost based on inverted index which is included in all the baseline methods.
When deployed into large-scale question answering systems, such as Google, our method can be greener than DENSPI.

\section{Conclusion}
In this paper, we present Ocean-Q, a novel method that uses QG to reduce the computational cost of RTQA, and address the bottleneck of encoding coming question which cannot be cached offline. 
Experiments on SQuAD-Open demonstrate that Ocean-Q is able to accelerate the fastest RTQA system by 4 times, while only losing the accuracy by 3+\%.
To further improve QG quality, we introduce a new data augmentation method and leverage multi-task learning and diverse beam search to boost RTQA performance.
%We also achieve state-of-the-art QG performance on HotpotQA.
Currently, there still exists a gap between Ocean-Q and the state-of-the-art RTQA models. 
Future work that includes designing a better QG model may help closing the gap.

==> Ocean-Q NAACL2021/intro.tex <==
\section{Introduction}
Real-time question answering (QA)~\cite{seo2018phrase,denspi} has enjoyed steadily growing attention in the community due to its commercial value in web-scale applications.
For practical use, QA search engines are required to return the answer given any real-time question within milliseconds in order to avoid human-detectable latency. So far, state-of-the-art QA models~\cite{devlin2018bert,liu2019roberta} rely heavily on cross-sequence attention between a given question and its relevant context in the document. Whenever a new question comes in, it needs to be encoded on the fly and attended to a list of relevant documents, which leads to considerable computational overhead especially when the given context is unlimited (\emph{e.g.}, open-domain setting).

To speed up the process, query-agnostic methods have been proposed to reuse question-related context for different questions.
\citet{seo2018phrase} proposed to build representations of key phrases only in the document and match them with the question representation to obtain answer.
\citet{denspi} further improved the quality of phrase embeddings and proposed a more effective way for caching.
However, the embeddings of incoming questions cannot be cached offline, which still leads to noticeable latency and additional cost of maintaining large neural networks in real applications. 

How can we efficiently reduce the energy cost while simultaneously speeding up real-time question answering for practical use? Here, we propose \textbf{Ocean-Q} (an \textbf{Ocean} of \textbf{Q}uestions), which removes the need of maintaining neural networks for real-time inference, and  significantly reduces question-encoding time in query-agnostic QA methods by leveraging high-quality offline question generation. The proposed pipeline consists of three steps: ($i$) Candidate Answer Extraction from the context; ($ii$) Question Generation based on the candidate answers; and ($iii$) QA-pair Verification by state-of-the-art QA models. Specifically, a candidate pool of all possible QA pairs is generated offline from the data corpus, and when a real-time question comes in, it is directly matched with the candidate pool via $n$-gram overlap to select the answer from the highest-ranked QA pair. 
%Note that our question generator is mainly trained on SQuAD dataset, we are not only generating frequently asked factoid questions.

\begin{figure*}[t!]
\centering
{\includegraphics[width=\linewidth]{images/ocean_q.png}}
\caption{\label{fig:overview} (a) is an overview of the Ocean-Q framework for real-time question answering, consisting of two components: Offline QA-pair Generation and Online Question Matching. Given a set of document paragraphs, steps of Answer Extraction, Question Generation and QA-pair Verification are applied sequentially to generate candidate QA pairs, which are cached into question ``ocean''. To efficiently search over the entire ocean, a two-step ranker is used during online question matching, and the question is then compared with the shortlist of QA pairs via instant $n$-gram matching to derive the right answer. Figures (b), (c) and (d) are used to further enhance Question Generation. Diverse Beam Search will penalize the node extended from the same parent node. QQP: Quora Question Pair dataset for duplicate question detection. SQuAD, HotpotQA, NewsQA: answer-extraction-based question answering datasets.}
\vspace{-10pt}
\end{figure*}

%The key ingredient of Ocean-Q is Question Generation (QG)~\cite{rus2008question, du2017learning, zhang-bansal-2019-addressing, unilm}, which has been widely studied in recent years.
%For example, offline-generated QA pairs are utilized in both semi-supervised and unsupervised QA systems~\cite{yang-etal-2017-semi, du-cardie-2018-harvesting,wang-etal-2019-adversarial-domain}.
%The evaluation of QG models commonly relies on BLEU~\cite{papineni2002bleu}, ROUGE~\cite{lin-2004-rouge} and METEOR~\cite{lavie2009meteor} scores. However, as discussed in~\citet{wang2018no}, these conventional metrics may not reflect the true quality of generated questions. 
To encourage more organic integration of Question Generation (QG)~\cite{rus2008question, du2017learning, zhang-bansal-2019-addressing, unilm} into QA systems, besides the QG evaluation metrics of BLEU~\cite{papineni2002bleu}, ROUGE~\cite{lin-2004-rouge} and METEOR~\cite{lavie2009meteor}, we also consider RTQA as a new quality criterion for QG models.
The symbiotical connection of QG and RTQA ensures end-to-end performance boost. In addition, we propose a new data augmentation approach and leverage multi-task learning and diverse beam search for QG enhancement to further improve RTQA performance.

%, and meanwhile speed up the real-time qa system by QG model.

%Our proposed method will address this issue by making full use of the QG system.

%\zhe{from the description below, it seems we should use RTQA as motivation, which is more appealing, and QG evaluation introduce later, rather than QG introduces first as it is now?}

%\paragraph{QG evaluation.}

%Since we could simply replace the QG-step in our Ocean-Q pipeline with any QG model, the end result of RTQA could be treated as a new means to measure intermediate QG performance.

%Specifically, we can simply replace the QG-step in our Ocean-Q pipeline with any QG model, then use the performance of RTQA as the metric for QG evaluation.\jj{What does this mean? Can we just say using the end result of RTQA model that leverages QG to measure intermediate QG performance?}
%To verify how well the new evaluation metric is, we further use data augmentation, multi-task learning and beam search strategies to boost the QG performance, and compare our evaluation method to BLEU and ROUGE scores.\jj{Why is this 'verifying' how well the metric is?}
%In more detail, we comprehensively explore how data augmentation, multi-task learning and beam search strategies can further boost the QG system.

Our main contributions are summarized as follows. 
($i$) We set up the first benchmark under the setting of answering open-domain questions without neural networks in real time. To the best of our knowledge, no previous work has leveraged question generation models to reduce the computational cost and mitigate the speed bottleneck in Real-time QA.
%($i$) We present Ocean-Q, a novel approach that leverages question generation models to mitigate the speed bottleneck in Real-time QA. 
($ii$) By generating possible candidate questions offline and circumventing real-time question encoding, Ocean-Q can successfully accelerate existing fastest RTQA system~\cite{denspi} by 4 times, with minimum accuracy drop, and make QA system greener by removing the cost of maintaining and running neural encoders. %\jj{Is the performance drop significant?} 
($iii$) We introduce a new data augmentation method and propose the use of multi-task learning and diverse beam search for QG quality enhancement that further boosts RTQA performance. %which could also be seen a new means to measure intermediate QG performance.
%to use RTQA as a new evaluation metric to assess and improve the quality of question generation, and conduct comprehensive experiments with three different methods for boosting QG performance. 
($iv$) Experiments show that our proposed approach achieves multifold speedup on generic QA models without sacrificing accuracy much. Our augmented QG component also achieves state-of-the-art performance on QG benchmarks of HotpotQA. %and on SQuAD.  
%We are the first to use the task of real-time question answering as an evaluation method for QG system;  ($ii$) We explore there types of methods to further boost the QG model and evaluate the methods by both Rouge/BLEU and question answering scores;  
%($iii$) We design a robust pipeline to generate a question and answer pool which can also be used for answering open-domain questions. 
%To the authors' best knowledge, this work is the first known effort to mutually enhance QG and RTQA with each other that achieves multifold speed-up on generic QA models without sacrificing accuracy much.

\section{Related Work}
\paragraph{Open-Domain Question Answering}
Open-domain QA aims to answer any given factoid question without knowing the target domain. 
%Methods in this field either use knowledge base or free-form text as the context.
We focus on text-based open-domain QA system~\cite{chen2017reading}, which first uses information retrieval (IR) to select passages, then applies a machine reading comprehension (MRC) model to extract answers from the passage pool.
%Since \citet{chen2017reading} built the first end-to-end system to tackle machine reading at scale, the IR phase has been investigated extensively \cite{wang2018r, kratzwald-feuerriegel-2018-adaptive, lee2018ranking, das2019multi, lee-etal-2019-latent, guu2020realm}.
%Meanwhile, MRC has also achieved great success in large-scale QA datasets, such as SQuAD~\cite{rajpurkar-etal-2016-squad}, especially after the advent of BERT~\cite{devlin2018bert}. 
Most works rely heavily on cross-sequence attention between questions and related context~\cite{yang2019end,raison2018weaver,wang-etal-2019-multi}, which translates to heavy online computational cost, since every related context needs to be processed repeatedly for a new input question. 
In order to reuse the context, \citet{seo2018phrase} proposed the phrase index QA task by encoding and indexing every possible text span offline into a dense vector.
DENSPI~\cite{denspi} further improved contextualized phrase embeddings with sparse vector, and designed effective caching strategies for real-time QA. 
%Very recently, ~\citet{lee2020contextualized} lifted DENSPI performance further by augmenting the sparse vector with contextualized information.
However, the shared bottleneck of all these works is the demanding time for encoding questions in real time execution.
In this paper, we propose to make full use of a QG-based RTQA framework that is able to achieve 4X speed-up without losing much accuracy.
\vspace{-5pt}

\paragraph{Question Generation}
Question generation was first proposed by \citet{rus2008question} as a task to automatically generate questions from given input. 
Since then, early work mainly focused on using manually designed rules or templates to transform input text to questions~\cite{heilman2011automatic, chali2012towards, lindberg2013generating}.
Due to the recent progress in deep learning, QG research started to adopt the prevailing encoder-decoder framework~\cite{serban-etal-2016-generating,du2017learning,du-cardie-2018-harvesting, liu2019learning, song2018leveraging, zhao-etal-2018-paragraph}.
%\citet{serban-etal-2016-generating} first used it to generate large-scale factoid QA pairs.
%\citet{du2017learning} then introduced attention-based sequence learning models for QG, consuming sentence-level input.
%Later on, some studies proposed to leverage direct or indirect information in paragraphs for QG~\cite{du-cardie-2018-harvesting, liu2019learning, song2018leveraging, zhao-etal-2018-paragraph}.
%To improve ``shallow'' questions that confine to a single sentence, deep QG has been explored~\cite{pan-etal-2020-DQG, gupta2020reinforced}.
More recently, large-scale language model pre-training has been applied to QG~\cite{unilm, unilmv2, xiao2020ernie}, which achieved state-of-the-art performance with significant improvement. 
Our QG method is based on the released UniLM model~\cite{unilm}, 
further improving it via novel data augmentation, multi-task learning and diverse beam search.
Moreover, to the best of our knowledge, we are the first work to connect neural question generator with real-time question answering.
\vspace{-5pt}

\paragraph{Green NLP} The primary focus of green NLP is to measure or reduce the amount of required computation to build effective models.
Green AI~\cite{schwartz2019green} covers a broader, long-standing interest in environmentally-friendly scientific research. With the success of pre-trained models~\cite{devlin2018bert} and large-scale datasets~\cite{deng2009imagenet,liu2019roberta}, efficient training and inference becomes increasingly critical regarding the green purpose. 
However, training time is relatively fixed comparing to real large-scale inference requirement, such as queries in Google search.
In this paper, we focus on addressing the green NLP problem regarding the inference efficiency of question answering systems. 
Model distillation~\cite{sun2019patient} or answer-embedding index~\cite{denspi} based methods are widely adopted to speed up the inference time.
However, these works still suffer from maintaining a large neural network to encode questions.
Instead, we propose to remove all the neural networks from the QA system. 
Thus, there will be little computational cost of answering questions, but only some information retrieval cost which can be quite efficient by reverted index. 

%\paragraph{QG Evaluation}
%Question generation evaluation has always been a challenge, since it is difficult to define a set of golden references.
%Semantic or syntactic correctness, fluency, ambiguity and diversity are all useful metrics, but subjective to define.
%Currently, most QG systems use human evaluation or automatic metrics for evaluation, such as BLEU~\cite{papineni2002bleu}, METEOR~\cite{lavie2009meteor} and ROUGE~\cite{lin-2004-rouge}. 
%In human evaluation, annotators are asked to rank generated questions, and the average rank or the percentage of best-ranked questions are used to evaluate model performance. 
%Some work also conducts pairwise comparison with baselines by asking annotators to provide binary judgement.
%Since human evaluation is time-consuming and small-scale, automatic metrics are widely adopted for evaluation.
%\citet{nema-khapra-2018-towards} proposed a so-called ``Q-metric'' to evaluate the answerability of generated questions. 
%\citet{zhang-bansal-2019-addressing} proposed to train a QA model on synthetic data only, and use the QA result as the evaluation for a QG model. 
%However, it is still an indirect metric that requires the QA model to be trained on synthetic data. 
%In this work, we consider the end result of RTQA score as a new quality criterion for intermediate QG performance, in order to connect QG with RTQA symbiotically.

==> Ocean-Q NAACL2021/model.tex <==
\section{Ocean-Q for Real-Time QA}
\label{sec:RTQA}

\subsection{Framework Overview}
\label{subsec:definition}
Our proposed approach to real-time question answering (RTQA) utilises QA pairs generated from a large-scale textual corpus (e.g., Wikipedia). 
The overview of the framework is illustrated in Figure~\ref{fig:overview}, consisting of two main components: ($i$) Offline QA-pair generation; and ($ii$) Online question matching. 

The QA-pair generation pipeline mainly consists of three steps: ($i$) Candidate answer extraction; ($ii$) Answer-aware question generation; and ($iii$) QA-pair verification.
First, we train an answer extraction model to create $K$ possible answer candidates $\{a_{i,j,k}\}_{k=0}^{K-1}$ from paragraph $p_{i,j}$ in document $d_i$. 
Then, for each candidate answer $a_{i,j,k}$, we generate $L$ diverse questions $\{q_{i,j,k,l}\}_{l=0}^{L-1}$ by combining $p_{i,j}$ and $a_{i,j,k}$ as the input of an answer-aware QG model. 
To further validate the generated QA pairs, a BERT-based QA model is utilized for authentication. 
By these three steps, we obtain approximately $N*M*K*L$ QA pairs from the whole Wikipedia, where $N$ is the number of documents, $M$ is the average number of paragraphs in a document, $K$ is the average number of answer candidates in a paragraph, and $L$ is the number of questions for each answer candidate. 
%generation \zhe{say in another way?}. 
With these pairs, the RTQA task is formulated as a ranking function $R$, where given an input question $\tilde{q}$, the goal is to predict the answer as $a=\arg\max_{i,j,k,l} R(q_{i,j,k,l}, \tilde{q})$.

\subsection{Offline QA-pair Generation}
\paragraph{Answer Extraction}
In principle, any span in a paragraph could be an answer candidate. 
To maintain high recall for QA, we formulate answer extraction as a classification problem and use pre-trained RoBERTa~\cite{liu2019roberta}.
For each token in the paragraph, we predict its probability of being the start and end position of the answer. Then, predicted answers with top-$K$ scores are selected as candidate answers.
Assume the encoded representation of a paragraph is denoted as  $\mathbf{C} \in \mathbb{R}^{n \times d}$, where $n$ is the length of the paragraph and $d$ is the dimension of each contextualized token representation. Then, the logits of every position being the start and end of the candidate answer span can be computed by a linear layer on top of $\mathbf{C}$:
\begin{align}
    \mathbf{o}_{s} = \mathbf{C}\mathbf{w}_{1},\,\,
    \mathbf{o}_{e} = \mathbf{C}\mathbf{w}_{2} \,,
\end{align}
where $\mathbf{o}_{s},\mathbf{o}_{e}\in \mathbb{R}^{n}$ and $\mathbf{w}_{1},\mathbf{w}_{2}\in \mathbb{R}^{d}$.
During training, the ground-truth distribution of a position being the start and end of an answer span is calculated over all possible answers in each paragraph, denoted as $P_s$ and $P_e$. 
A KL divergence loss is then defined as:
\begin{equation}
    \mathcal{L} = D_{KL}(P_{s}||Q_{s}) +  D_{KL}(P_{e}||Q_{e})\,,
\end{equation}
where $Q_s$ and $Q_e$ are the predicted distributions of a position being the start and end of an answer span based on the logits $\mathbf{o}_{s}$ and $\mathbf{o}_{e}$.
%$P_s$ and $P_e$ are the ground truth distribution for start and end position.
During inference, we first calculate the start and end logits for each token in the paragraph, then top-$K$ answer spans are extracted based on the score below:
\begin{equation}
    s_k = \mathbf{o}_{s}[a_{s,k}] + \mathbf{o}_{e}[a_{e,k}]\,,
\end{equation}
where $s_k$ is the score for the $k$-th answer candidate $a_k$ with start and end position being $a_{s,k}$ and $a_{e,k}$.
%(assume the start and end of the answer span is ) of each that ranges from $k_s$ to $k_e$

%In our system, We limit the maximum answer length as 10 and take top 100 candidate answers. \zhe{why not use rule-based system to extract answers?}

\paragraph{Question Generation}
For question generation, we build upon the released state-of-the-art UniLM model~\cite{unilm}. 
To generate $L$ different questions given an answer span, we adopt standard beam search strategy.
More formally, we concatenate a given input passage $p_{i,j}$ and an answer span $a_{i,j,k}$ as the first segment (denoted as $X$), and incrementally generate each token of the target question.
At time step $t-1$, the model keeps track of $L$ hypotheses and their scores $S(q_{t-1}|X)$, where $L$ is the beam size and $q_{t-1}$ is a generated token. 
Then, at time step $t$, each hypothesis selects $L$ extensions, which leads to $L*L$ hypotheses in total.
%The score of each new hypotheses is:
%\begin{align} \label{equ:standard-beam}
%    \mathbf S(q_{t-1}^k, q_{t}^{k,k^{\prime}}|X) &= S(q_{t-1}^k|X) %\nonumber \\
%    &+ \log p(q_{t}^{k,k^{\prime}}|X; q_{t-1}^k)
%\end{align}
In the end, the top-$L$ generated questions are selected from $L*L$ hypotheses at the final time-step $T$. We further explore different strategies to improve QG model, detailed in the Enhanced Question Generation Section. %~\ref{sec:qg_eval}.
%\zhe{the above equation seems not needed. standard beam search.}

\paragraph{QA-pair Verification}
With the aforementioned two steps, we can obtain an initial set of QA pairs.
However, these answers may not be accurate enough since answer extraction model could not precisely know where is the answer boundary.
% Not a good example
For example, the extracted span ``February 7 '' might be a sub span of the gold answer ``February 7, 2016'' which leads to a lower RTQA performance.
%\jj{Why lower?}
Therefore, we use the initial QA dataset to train a BERT-based QA model, to validate the initial QA pool.
Then, we replace the the initial answer $a_{i,j,k}$ with the predicted answer $a_{i,j,k}^{\prime}$ from the QA model.
%\begin{equation}
%    \sum_{\langle p, q, a \rangle \in D_1} \log P(a|p,q)
%\end{equation}

\subsection{Online Question Matching}
The main challenge in real-time question matching is how to efficiently search over the entire question ``ocean'' that consists of $N*M*K*L$ questions. 
Given that the ranking function $R$ can be a simple scoring function, the problem can be redefined as finding accurate paragraphs among $N*M$ paragraphs that may lead to the correct answer. Therefore, we propose a two-step ranker and conduct question matching as follows.

\paragraph{A Two-step Ranker}
DrQA~\cite{chen2017reading} has demonstrated strong capability in finding relevant documents based on bi-gram hashing and TF-IDF matching.
Therefore, we leverage DrQA to build a document-level TF-IDF sparse vector $\mathbf{d}_i$ for each document. 
The input question is also encoded into a bi-gram TF-IDF sparse vector $\mathbf{q}$. 
Then, top-$n$ documents are retrieved from $N$ documents by calculating the inner product between $\mathbf{q}$ and each $\mathbf{d}_i$.
Similarly, we also compute a second paragraph-level TF-IDF $\mathbf{p}_i$ for each paragraph after the first ranker, and collect top-$m$ paragraphs only based on the inner product score on paragraph-level.
Since paragraphs capture more local information than documents, by implementing the two-step ranker, we can safely reduce the number of paragraphs from $N*M$ to $m$ ($m \ll N*M$) for question ranking in the final step.

\paragraph{Question Matching}
After the proposed two-step ranking process, the total number of candidate questions reduces to $m*K*L$ (around 200k, if $m,K,L$ are $100, 100, 20$, respectively).
We simply calculate the common number of unique tokens to measure the similarity between each question candidate $q_i$ and the input question $\tilde{q}$. Specifically,
\begin{equation}
    score(\tilde{q}, q_i) = \frac{\tilde{\mathbf{q}}\cdot \mathbf{q}_i}{|\tilde{\mathbf{q}}| + |\mathbf{q}_i|}\,,
    %score(q, q_i) = \sum_{t \in q} \frac{freq(t,q)}{\sum_{t^{\prime} \in q_i} freq(t^{\prime}, q)}
\end{equation}
where $\tilde{\mathbf{q}}$ and $\mathbf{q}_i$ are binary sparse representations, indicating whether each token in the vocabulary exists in the question or not. $|\tilde{\mathbf{q}}|$ and $|\mathbf{q}_i|$ are the $\ell_1$ norm of each vector. After question matching, we use the corresponding answer to the retrieved question as the final predicted answer. 

\subsection{Enhanced Question Generation}
\label{sec:qg_eval}
Question Generation is a critical component in Ocean-Q framework. We hypothesize that more diverse questions from QG model may enhance the RTQA performance.
To verify this, we investigate from three perspectives: ($i$) we propose a new data augmentation method to increase in-domain training data diversity; ($ii$) we leverage multi-task learning with out-of-domain training data; ($iii$) we leverage diverse beam search in decoding phase.
%Besides, the final RTQA store can be viewed as a new means for evaluating intermediate QG models since we can simply replace the QG module in the Qcean framework with any QG model
%Current QG evaluation mostly relies on standard text generation metrics such as BLEU, ROUGE and METEOR.
%However, these metrics often fail to directly reflect QG effectiveness in downstream tasks.
%Since we can simply replace the QG module in the Qcean framework with any QG model, the final RTQA store then can be viewed as a new metric for evaluating QG models. In this section, we investigate three different methods to enhance QG for better Qcean performance. \jj{Should we mention that MTL and beam search have been explored before, and our main contribution is augmentation and the combination of all three?} At the same time these methods are used to verify whether the RTQA score is a good metric for QG evaluation. \jj{This is confusing. How to use these three methods to verify how good a metric is?}

\paragraph{Data Augmentation}
To increase the diversity of the QG training dataset $D_1$, we select additional samples from the generated question pool and reuse them as training data. 
A caveat is that the generated questions may semantically diverge from the original question, so we aim to select only a small portion from the pool to augment the training data. %\jj{Does this ensure the avoidance of the caveat?}
To this end, we train a question paraphrasing model on the Quora Question Pairs (QQP) dataset\footnote{https://www.quora.com/q/quoradata/First-Quora-Dataset-Release-Question-Pairs} $D_2$ to obtain a paraphrase score between the generated question and the ground-truth question, and use it as one of the guidelines for question selection.
Moreover, since semantically-similar questions may overlap with each other, we also use the $F_1$ metric to calculate the number of overlapping tokens between the generated question and the ground-truth question as another guideline.
Thus, for each data sample in $D_1$, we can effectively craft augmented training samples, forming a new dataset $D_3$, and the final QG model $M_{QG}^{\prime}$ is trained by combining $D_1$ and $D_3$. 
The proposed data augmentation method is summarized in Algorithm~\ref{alg:DataAugmentation}.

\paragraph{Multi-task Learning}
Multi-task learning (MTL) \cite{caruana1997multitask} has been proved to be effective for improving model generalization.
However, directly mixing all the tasks has the potential downside of biasing the model towards auxiliary tasks instead of the intended target task. 
Therefore, \citet{xu-etal-2019-multi} proposed a mixed ratio strategy and verified its effectiveness in MRC tasks.
Inspired by this, we apply the MTL algorithm to QG:
given $K$ different tasks and $D_1$ as the target task, we use all mini-batches from $D_1$ and sample specified ratio of mini-batches from the remaining tasks.
In experiments, we use hyper-parameter search to find the best ratio for each target task.

\begin{algorithm}[t!]
\small
\caption{\label{alg:DataAugmentation}Data Augmentation for QG.}
\SetAlgoNoLine
\SetArgSty{}
\KwIn{QG dataset $D_1$, QQP dataset $D_2$, QQP score threshold $s_{min}, s_{max}$, $F_1$ score threshold $f_{min}, f_{max}$, maximum selection number $N$}
 Train QG model $M_{QG}$ on $D_1$\;
 Train QQP model $M_{QQP}$ on $D_2$\;
 $D_3$ = \{\}\;
 \ForEach{$ \langle p,q,a \rangle \in D_1$}{
    Generate $L$ different questions with beam search 
    $q_1, .., q_L = M_{QG}(p,a)$\;
    Calculate QQP score for each question
    $s_{qqp}^{i}=M_{QQP}(q_i, q), 1 \le i \le L$\;
    Calculate $F_1$ score for each question
    $s_{f1}^{i}=F_1(q_i, q), 1 \le i \le L$\;
    $D_{sel}$ = \{\}\;
    \For{$i=1$ \KwTo $L$}{
        \If{$s_{min} \le s_{qqp}^{i} \le s_{max} $ and 
            $f_{min} \le s_{f1}^{i} \le f_{max} $ and 
            $len(D_{sel}) \le N$}{
        add $\langle p,q_i,a \rangle$ to $D_{sel}$
        }
    }
    add $D_{sel}$ to $D_3$ \;
  }
  Train QG model $M_{QG}^{\prime}$ on $D_1$ and $D_3$ \;
\KwOut{$M_{QG}^{\prime}$}
\end{algorithm}

\paragraph{Diverse Beam Search}
%Asking questions based on a given answer is a ``one-to-many'' mapping problem.
%However, BLUE and ROUGE scores by nature fail to evaluate the diversity of generated questions, while diversified questions may be beneficial for downstream QA task.
%To this end, we adopt the diverse beam search strategy~\cite{li2016simple} to further enhance QG model.
Standard beam search tends to generate similar sequences in the $n$-best list. 
To mitigate this, \citet{li2016simple} proposed to penalize the hypotheses that are extended from the same parent node, effectively favoring outlets from more diverse parents.
In our work, we leverage this directly to generate more diverse questions for each candidate answer.
More formally, the score for each question hypothesis is written as:
\begin{equation}
    S(q_{t-1}^k, q_{t}^{k,k^{\prime}}|X) = S(q_{t-1}^k, q_{t}^{k,k^{\prime}}|X) - {\gamma}k^{\prime}\,,
\end{equation}
where $X$ is the context, $q_{t-1}^k$ is the $(t-1)$-th generated token at beam $k$, $q_{t}^{k,k^{\prime}}$ is the $t$-th generated token at beam $k^\prime$ based on $q_{t-1}^k$, $k^{\prime}$ is the rank of the current hypothesis among its siblings, and $\gamma$ is the diversity rate. $S(q_{t-1}^k, q_{t}^{k,k^{\prime}}|X)$ is the ranking score used in standard beam search. In experiments, we show that using diverse beam search can effectively improve RTQA performance.%, even with sacrificed performance on conventional metrics such as BLEU and ROUGE.
